Conversation Derailment Forecasting with Graph Convolutional Networks

Online conversations are particularly susceptible to derailment, which can manifest itself in the form of toxic communication patterns like disrespectful comments or verbal abuse. Forecasting conversation derailment predicts signs of derailment in advance enabling proactive moderation of conversations. Current state-of-the-art approaches to address this problem rely on sequence models that treat dialogues as text streams. We propose a novel model based on a graph convolutional neural network that considers dialogue user dynamics and the influence of public perception on conversation utterances. Through empirical evaluation, we show that our model effectively captures conversation dynamics and outperforms the state-of-the-art models on the CGA and CMV benchmark datasets by 1.5\% and 1.7\%, respectively.

==> introduction-old.tex <==
\section{Introduction}

Popularity of social media leads to huge volumes of online conversations, some positive, others not. 

Social media are rife with hate speech. Conversations in social media can derail when participants become hostile and attack each other. Hate speech and toxic communication online has become a serious and prevalent problem \cite{thirty}, a quick glance at the comments section of controversial posts  demonstrates how prevalent the problem is. Generally,  social media companies  self-regulate by providing human moderators \cite{virtual}. The burden on human moderators has motivated research in assisting computational approaches.

 
 
\begin{table}[t!]
%\small
\centering
\resizebox{\columnwidth}{!}{

\begin{tabular}
{ccp{5cm}c}
\toprule
\textbf{turn} & \textbf{user} & \textbf{text} & \textbf{label}\\  
\midrule
$N-3$  & $\mathcal{A}$ & {\em ``Proper use of an editor's history includes  fixing errors or violations of Wikipedia policy or correcting related problems on multiple articles." } &   \\
$N-2$ & $\mathcal{B}$ & {\em  ``All you are doing is following me round the biography articles  it's very clear that you just go to my contributions list and look to see what biography articles I've worked on, then you go and look to see if you can find something wrong with them.  
" } & \\
$N-1$ & $\mathcal{A}$ & {\em  ``So, what is wrong with fixing things? At the top of my talk page, it says to keep it on your watchlist. "} & \\
$N$ & $\mathcal{B}$ & {\em  ``You cannot possibly be too stupid to understand the warning I'm giving you.  I'm not going to repeat it."}  & \textbf{\textcolor{red}{???}}\\
\bottomrule
\end{tabular}
}

\caption{A sample conversation from the Conversation Gone Awry dataset showing a sequence of text utterances that end with a verbal abuse. Given the conversation context upto $N-1$ turns, the task is to predict whether turn $N$ will be a respectful or offensive statement leading to derailment (\textcolor{red}{it is offensive}, in this case).}
\label{tab:example}
\end{table}
Research on computational approaches in this area has mostly focused on detecting antisocial behavior after the fact. These approaches analyze single comments in isolation.  This stands in opposition to forecasting derailment, that aims to predict  hostile behavior between users in online conversations before it happens. That is, to provide timely notice  to human moderators of a potential conversation derailment before it occurs. When forecasting, the earlier the warning for a potential derailment comes, the more actionable it is.

Approaching such conversational forecasting problems, however, requires overcoming inherent modeling challenges. Conversations are dynamic and their outcome might depend on how subsequent comments interact with each other, who are interacting with each other and the effect of public perception on the comments made in the conversation. 
 
There exist two datasets used in the literature  for the purpose of research on forecasting online conversation derailment. These datasets are Conversations Gone Awry (CGA)\cite{CGA} and Reddit ChangeMyView (CMV)\cite{cmv}. Both these datasets contain  conversations between multiple participants annotated with a label on whether they will derail or not. They both contain the textual input and user ID for each of the utterances in the conversation, CMV also includes a public vote on each of the utterances in the conversation.  Table \ref{tab:example} shows an example conversation from the CGA dataset that derails. As can be seen in the example,  the personal nature of the attack asks if textual information in isolation  of user information can best capture if a conversation  would derail. There could also be a history between the two users from previous conversations. 

Current work in online conversational derailment forecasting has focused solely on the textual input and in the sequence of a conversation.  Figure \ref{fig:example}  shows an example conversation structure found in CGA that is not sequential in nature and contains multiple users where a number of users  are in agreement and not part of the heated exchange.  Relational graphs would better represents the actual structure and user dynamic in such  conversations. Figure \ref{fig:examplecmv}  shows and example conversation in CMV. In addition to distinct regions of argument within the conversation, CMV contains public voting scores on each turn in the conversation that may contain patterns that relate to derailment. 

Graph neural networks have been used to model conversations for the purpose of classification. For example, they have shown promise in forecasting the next emotion in a conversation, a problem  similar to that of interest in this work. This motivated us to  explore this line of research with the following contributions:
\begin{itemize}
    \item we propose  \textcolor{red}{ a new {\em  graph convolutional network model}, the Forecasting Graph Convolutional Network (FGCN),} that incorporates  textual, user and public perception data.
    \item we perform an extensive empirical evaluation of the proposed model across two datasets and provide a thorough report of the analysis that can inform adoption of the model in real scenarios and diverse applications.
        \item we (aim to) make source code publicly available to encourage reproducibility.
\end{itemize}
% Organization of the paper
The remainder of the paper is organized as follows. Section \ref{sec:related} reviews the related work. The technical problem of interest in this paper is presented in Section \ref{sec:problem}. Our proposed models are introduced in Section \ref{sec:models}.  Section~\ref{sec:experiments} presents an experimental evaluation of the different models, the results and discussion are in Section \ref{sec:results}, and the conclusions are presented in Section~\ref{sec:conclusions}.





\begin{figure}[t]
     \centering
     \begin{subfigure}[b]{0.19\textwidth}
         \centering
         \includegraphics[width=\textwidth]{conv2.jpg}
         \caption{Conversation $C_{CMV}$}
         \label{fig:examplecmv}
     \end{subfigure}
     \begin{subfigure}[b]{0.28\textwidth}
         \centering
         \includegraphics[width=\textwidth, height=5.4cm]{conv1.jpg} 
         \caption{Conversation $C_{CGA}$}
         \label{fig:example}
     \end{subfigure}

\caption{Example conversation structures from two datasets. a shows an example conversation  $C_{CMV}$ from the CMV  dataset and b shows an example conversation  $C_{CGA}$ from the CGA  dataset. }

\label{fig:cm}
\end{figure}
